The Effects of Linear Matter Power Spectrum Enhancement on Dark Matter Substructure

We present cosmological dark matter (DM)--only zoom-in simulations of a Milky Way analog originating from enhanced linear matter power spectra $P(k)$ relative to the standard cold, collisionless DM (CDM) cosmology. We consider a Gaussian power excess in $P(k)$ followed by a cutoff in select cases; this behavior could arise from early-Universe physics that alters the primordial matter power spectrum or DM physics in the radiation-dominated epoch. We find that enhanced initial conditions (ICs) lead to qualitative differences in substructure relative to CDM. In particular, the subhalo mass function (SHMF) resulting from ICs with both an enhancement and cutoff is amplified at high masses and suppressed at low masses, indicating that DM substructure is sensitive to features in $P(k)$. Critically, the amplitude and shape of the SHMF enhancement depend on the wavenumber of the $P(k)$ excess and the presence or absence of a cutoff on smaller scales. These alterations to the SHMF are mainly imprinted at infall rather than during tidal evolution. Additionally, subhalos are found systematically closer to the host center, and their concentrations are increased in scenarios with $P(k)$ enhancement. Our work thus reveals effects that must be captured to enable $P(k)$ reconstruction using DM substructure.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

